Negative Token Merging: Image-based Adversarial Feature Guidance

Text-based adversarial guidance using a negative prompt has emerged as a widely adopted approach to steer diffusion models away from producing undesired concepts. While useful, performing adversarial guidance using text alone can be insufficient to capture complex visual concepts or avoid specific visual elements like copyrighted characters. In this paper, for the first time we explore an alternate modality in this direction by performing adversarial guidance directly using visual features from a reference image or other images in a batch. We introduce negative token merging (NegToMe), a simple but effective training-free approach which performs adversarial guidance through images by selectively pushing apart matching visual features between reference and generated images during the reverse diffusion process. By simply adjusting the used reference, NegToMe enables a diverse range of applications. Notably, when using other images in same batch as reference, we find that NegToMe significantly enhances output diversity (e.g., racial, gender, visual) by guiding features of each image away from others. Similarly, when used w.r.t. copyrighted reference images, NegToMe reduces visual similarity to copyrighted content by 34.57%. NegToMe is simple to implement using just few-lines of code, uses only marginally higher (<4%) inference time and is compatible with different diffusion architectures, including those like Flux, which don't natively support the use of a negative prompt. Code is available at https://negtome.github.io

==> sec/0_abstract.tex <==

% \ranjay{This is a really weak way to begin a paper. You are saying that something has emerged and that you provide an alternative option. This framing doesn't mention the impact of either options.}
% \pw{+1. We should describe the problem we're trying to solve, why it's not yet solved by existing methods, and what's the key idea behind our method that lets us solve it.} \pw{Also missing from the abstract is what we apply this to and the results contextualized against prior art}
Text-based adversarial guidance using a negative prompt has emerged as a popular approach in order to push the output features away from undesired concepts. In this paper, for the first time we explore an alternate modality in this direction by performing adversarial guidance directly using visual features from a reference image or other images in a batch. In particular, we introduce negative token merging (\negtome), a simple but effective training-free approach which performs adversarial guidance by selectively 
    % finding and 
    pushing apart matching semantic features (between reference and output generation) during the reverse diffusion process. When used w.r.t.~other images in the same batch, we observe that \negtome significantly increases output diversity (racial, gender, visual) without sacrificing output quality. Similarly, when used w.r.t.~a reference copyrighted image asset, we observe that \negtome helps reduce visual similarity with copyrighted content by 34.57\%. \negtome is simple to implement using just few-lines of code and generalizes to different 
    diffusion architectures like Flux, which do not natively support the use of a separate negative prompt.
    % \swj{motivate a bit more why we need image-based adversarial guidance. how it is better than text based one? it would be helpful to clarify specific applications or scenarios where image-based guidance is essential while text-based one cannot work.} \linjie{This is exactly our struggle. It is hard to find a case that text-based ones cannot work. Copyright mitigation is the scenario, but if the character is not famous, the character cannot be generated by the model. I think our goal is not to completely replacing text-based adversarial guidance. Even for the diversity case, we are not completely replacing existing method (e.g., prompt rewriting). It can be used together with these text-based methods. }
    
    % helps better reduce copyright violation as opposed to traditionally used negative prompt. Furthermore, 
    % we find that 
    % NegToMe is model-agnostic and applicable to different diffusion architectures like Flux which do not natively support the use of a separate negative prompt.
    % while on avg while on average showing comparable inference times.


